New directions for surrogate models and differentiable programming for High Energy Physics detector simulation

The computational cost for high energy physics detector simulation in future experimental facilities is going to exceed the current available resources. To overcome this challenge, new ideas on surrogate models using machine learning methods are being explored to replace computationally expensive components. Additionally, differentiable programming has been proposed as a complementary approach, providing controllable and scalable simulation routines. In this document, new and ongoing efforts for surrogate models and differential programming applied to detector simulation are discussed in the context of the 2021 Particle Physics Community Planning Exercise (`Snowmass').

==> ongoing_rewrite.tex <==
% NOW OBSOLETE: relevant changes integrated in main document

% rephrasing of last para of introduction
This document is divided as follows. Sections~\ref{sec:works} and \ref{sec:diffprog} present brief introductions to surrogate models based on ML techniques and differentiable programming. In Secs.~\ref{sec:contrib:EK_WH}, \ref{sec:contrib:CK}, and \ref{sec:contrib:MK}, several ongoing projects are described and discussed. These examples are not meant to be comprehensive, but instead illustrative of the scope of research in this area. Finally, in Sec.~\ref{sec:future}, future directions and synergies in the short and long term future are explored.

\section{Surrogate Models}\label{sec:works}

% taken from the footnote in the current introduction
The existing landscape of detector simulation consists of two primary approaches. The first is the accurate, but computationally intensive ``full simulation'' using \geant. The second is typically called ``fast simulation'' and may be considered a classical version of a surrogate model. Decreased simulation time is achieved by replacing computationally intensive parts of the simulation with simplified detector assumptions, resulting in speed improvements of more than 100 times compared to the full simulation. The resulting simulation, however, is less realistic and may be unsuitable for physics measurements that rely on detailed detector effects. Within the category of classical fast simulation, there are experiment-specific solutions~\cite{ATLAS:2010arf,Sekmen:2016iql} and the ultra-fast generic simulation \delphes~\cite{deFavereau:2013fsa}. Figure~\ref{fig:ml4sim_diagram} shows the different ways to introduce ML to this landscape: by replacing or augmenting part or all of \geant, or part or all of a classical fast simulation. Each option has a different goal: increasing speed while preserving accuracy, or preserving speed while increasing accuracy, respectively.

\begin{wrapfigure}{l}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{ML4Det/figures/ml4sim_diagram.pdf}
    \caption{Depiction of different ways to incorporate ML in detector simulation workflows.} 
    \label{fig:ml4sim_diagram}
\end{wrapfigure}

Alternatively, different ML surrogate models approaches may be classified based on what input data they require to produce simulated events. This leads to two categories: 1. fully generative models that entirely replace classical simulation engines, taking generated particle data or random noise as input; and 2. refinement techniques that are applied during or after the event simulation step, taking lower-quality simulated events as input. Popular deep learning architectures for fully generative models are divided into three main categories including generative adversarial networks (GANs) \cite{Paganini:2017hrr,Paganini:2017dwg,deOliveira:2017rwa,DiSipio:2019imz,Farrell:2019fsm,Erdmann:2018kuh,Erdmann:2018jxd,Deja:2019vcv,Musella:2018rdi,Vallecorsa:2018zco,Carminati:2018khv,ATL-SOFT-PUB-2018-001,Chekalina:2018hxi,SHiP:2019gcl,Martinez:2019jlu,Butter:2020tvl,2009.03796,Kansal:2020svm,Maevskiy:2020ank,Choi:2021sku,Rehm:2021zow,Rehm:2021zoz,Kansal:2021cqp,Khattak:2021ndw,Bravo-Prieto:2021ehz,ATLAS:2021pzo}, variational autoencoders (VAEs) \cite{ATL-SOFT-PUB-2018-001,Buhmann:2021lxj,Hariri:2021clz,Mu:2021nno,Orzari:2021suh}, and normalizing flows \cite{Lu:2020npg,Krause:2021ilc,Krause:2021wez, Butter:2021csz}. Refinement techniques may be based on classification \cite{2009.03796,Winterhalder:2021ave} or regression \cite{Chen:2020uds,banerjee2022denoising}. The generative models apply a stochastic approach, while the refinement techniques are usually deterministic.

Initially proposed in \cite{NIPS2014_5ca3e9b1}, GANs are trained following a minimax game:
\begin{equation}
    \min_{G}\max_{D}V(D,G) =  \mathbb{E}_{x\sim p_x(x)}[\log D(x)] + \mathbb{E}_{z\sim p_z(z)}[\log(1-D(G(z)))]\,,     
\end{equation}
where a generator network $G$ is tasked to generate new samples from a noise distribution $p_z(z)$ while the discriminator network $D$ judges the quality of the generated samples by comparing with target events sampled from $p_x(x)$. The adversarial loss function can lead to unstable training, often requiring additional fine tuning to achieve realistic results. An alternative to the loss function was proposed in Ref.~\cite{arjovsky2017wasserstein}, called Wasserstein GAN (WGAN). In the WGAN framework, the discriminator network is replaced with a critic network that uses the Wasserstein distance between generated and data samples as a metric to be minimized during training. There are many GAN variations that go beyond the vanilla and WGAN approaches.

Autoencoders are composed of two components: an encoder that compresses a set of input features into a smaller latent space, and a decoder that uses the information in that latent space to attempt to reconstruct the input features. VAEs combine autoencoders with a tractable latent space to generate new and realistic samples. Even though the probability density of the data is not tractable, VAEs minimize the evidence lower bound loss:

\begin{equation}
    \mathcal{L}_{\mathrm{VAE}} = -\mathbb{E}_{z\sim q(z|x)}[\log p_x(x|z)] + \mathcal{D}_{KL}(q(z|x)||p_z(z)).
\end{equation}
%
The approximate posterior probability density $q(z|x)$ is enforced to be a tractable  distribution through the Kullback–Leibler  divergence term $\mathcal{D}_{KL}$. The reconstruction loss $\log p_x(x|z)$ is often defined as the mean squared error loss, in case of continuous distributions, or the cross-entropy loss, in case of discrete distributions.

As an alternative approach to handling data with an intractable probability distribution, normalizing flows~\cite{2015arXiv150505770J,2019arXiv190809257K,2019arXiv191202762P} define a bijective transformation between a tractable base distribution, such as a normal or uniform distribution, to the data using the transformation of variables:

\begin{equation}
    \log{p_{x}(x)} =  \log{p_{z}(z)} -\log\mathrm{det}\left| \frac{\partial f(z)}{\partial z}\right|,
    \label{eq:flow}
\end{equation}
%
with terms $\frac{\partial f(z)}{\partial z}$ representing the Jacobian matrix of the transformation $f$. The loss function to be minimized is then defined as $-\log{p_{x}(x)}$, which is equivalent to minimizing the KL divergence between the transformed tractable base distribution and the data distribution.

The general calculation of the determinant in Eq.~\ref{eq:flow} has $\mathcal{O}(D^3)$ computational cost. This limitation is mitigated by restricting the bijective transformation $f$ to the family of functions with triangular Jacobian matrix, bringing the computational complexity down to $\mathcal{O}(D)$. 
There exist two main architectures to ensure a triangular Jacobian: bipartite~\cite{2016arXiv160508803D} flows based on so-called coupling layers or autoregressive~\cite{2017arXiv170507057P,2016arXiv160604934K} flows based on masked neural networks (NNs)~\cite{2015arXiv150203509G}. Practically speaking, their main difference is the speed in which both directions of the bijector can be evaluated. In bipartite flows accessing the log-likelihood of data and sampling is equally fast. Autoregressive flows have a fast and a slow direction. Masked Autoregressive Flows (MAFs)~\cite{2017arXiv170507057P} are fast in density estimation, but a factor $D$, given by the dimension of data space, slower in sampling. Inverse Autoregressive Flows (IAFs)~\cite{2016arXiv160604934K} are fast in sampling, and a factor $D$ slower in estimating the density of data points. See~\cite{2019arXiv190809257K,2019arXiv191202762P} for more details on normalizing flows.
An application of density estimation for calorimeter simulation is described in Sec.~\ref{sec:contrib:CK}. A simplified depiction for the different generative strategies is shown in Fig.~\ref{fig:gan_chart}.

\begin{wrapfigure}{l}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{ML4Det/figures/Gen_chart.pdf}
    \caption{Summary of different machine learning methods used for generative models.} 
    \label{fig:gan_chart}
\end{wrapfigure}

A natural question about surrogate models is to what extent the generated samples increase the statistical power with respect to the training data~\cite{Matchev:2020tbw}. At its core, the benefit from deep generative models comes from their ability to interpolate in high dimensions. One source of statistical amplification from the training dataset is from combinatorics - there are combinatorially many ways to attach showers to $N$ particles in an event and deep generative models can naturally interpolate from the training dataset to have the correct kinematic properties.  Interpolation also can result in precise statisical properties from ...~\cite{2008.06545,Bieringer:2022cbs}

Further refinements to generated samples can be derived to improve generation quality. Those corrections can be coupled either to ML-based surrogate models or to classical fast simulation routines. Advantages of refinement in the former case include that the training is often more stable than for the original generative model, and correspondingly, the generative model may not need to match the precision of \geant. Alternatively, replacing the generative model with a classical simulator and relying on ML only for refinement may decrease the probability of unphysical output and provide better extrapolation beyond the training data. Some example applications of this type are discussed in Sec.~\ref{sec:contrib:EK_WH}.

\section{Differentiable Programming}\label{sec:diffprog}

An alternative but complementary direction for surrogates lies in recent advancements in differentiable programming (DP).  In DP, software is written in, or transformed into, differentiable code via the use of automatic differentiation (AD)~\cite{autodiff}, an algorithmic way to efficiently evaluate derivatives of computer programs. When software is written in DP frameworks, access to the dependence of predictions on inputs is enabled through gradients. 

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{ML4Det/figures/diff_prog.pdf}
    \caption{An illustration of differentiable programming for detector simulation.} 
    \label{fig:diff_chart}
\end{wrapfigure}

These gradients are a significant addition to the information typically provided by simulators and crucially can be used in downstream modeling and inference tasks. This approach is flexible and optimizable; differentiable HEP software and ML tools can be mixed, for instance to use ML surrogates of non-differentiable computations, and can be jointly optimized to improve speed and prediction accuracy. When developed with DP, HEP simulation tools, and the physics knowledge they encode, can be used as physics prediction engines directly within ML pipelines for developing physics-informed ML tools. An illustration of differentiable programming is shown in Fig.~\ref{fig:diff_chart}. We note that deep generative models are a type of differentiable detector simulation, since gradients are readily available for neural networks. More details on differentiable programming for detector simulation are given in Sec.~\ref{sec:contrib:MK}.
